Estimating Idea Production: A Methodological Survey

Accurately modeling the production of new ideas is crucial for innovation theory and endogenous growth models. This paper provides a comprehensive methodological survey of strategies for estimating idea production functions. We explore various methods, including naive approaches, linear regression, maximum likelihood estimation, and Bayesian inference, each suited to different data availability settings. Through case studies ranging from total factor productivity to software R&D, we show how to apply these methodologies in practice. Our synthesis provides researchers with guidance on strategies for characterizing idea production functions and highlights obstacles that must be addressed through further empirical validation.

==> archived/main_v2_archive.tex <==
\subsubsection{Results}

We choose to use the model from Section \ref{sec:third-proposal} with \( X_p \) restricted to be a drift-diffusion process, as this process has the most realistic noise structure in the case \( \lambda = 0 \). In this case, as explained in Section \ref{sec:third-proposal}, we're able to leverage the explicit forward probability densities from \cite{roodman2020probability} to provide the log-likelihoods necessary for a Bayesian update.

The choice of priors is also fairly important. Recall Equation \ref{eq:third-proposal-gaussian-law-of-motion-two}:

\begin{equation}
\tag{\ref{eq:third-proposal-gaussian-law-of-motion-two} revisited}
    \frac{dA}{A} = \theta A^{-\beta} I^{\lambda} \, dt + \sigma A^{-\beta/2} I^{\lambda/2} \, dW_t
\end{equation}

Of the four parameters of this SDE, \( \beta, \lambda \) are dimensionless and we pick independent half Cauchy priors with unit scale over both of them. However, the situation is not as straightforward for the remaining parameters \( \theta, \sigma \), as these two parameters have complicated dimensions. Using square brackets to denote dimensions, we have \( [\theta A^{-\beta} I^{\lambda} \, dt] = 1 \) and so \( [\theta] = [A]^{\beta} [I]^{-\lambda} [t]^{-1} \). Similarly, \( [\sigma] = [\theta]^{1/2} = [A]^{-\beta/2} [I]^{\lambda/2} [t]^{-1/2} \). This is suggestive that we should find some scales \( A_s, I_s, \Delta t_s \) and then pick half Cauchy priors with unit scale over the two dimensionless quantities

\begin{align}
\label{eq:dimensionless-constants}
    \theta_s &= \theta A_s^{-\beta} I_s^{\lambda} (\Delta t_s) \\
    \sigma_s &= \sigma A_s^{-\beta/2} I_s^{\lambda/2} (\Delta t_s)^{1/2}
\end{align}

We make the choices \( A_s = A_{\text{initial}}, \, I_s = I_{\text{initial}}, \, \Delta t_s = (t_{\text{final}} - t_{\text{initial}})/\log(A_{\text{final}}/A_{\text{initial}}) \). This normalization has the advantage that it's scale-invariant: changing the units of \( A, I \), or \( t \) doesn't change the results we obtain from the estimation. There are other scale-invariant normalizations as well, but we think our choice is the most natural one. Our final priors are therefore \( \lambda, \beta, \theta_s, \sigma_s \sim \text{HalfCauchy}(1) \) with the priors for all four dimensionless parameters being jointly independent. It is possible to be more aggressive by choosing a prior that is more strongly bounded away from zero and infinity, but we stick to Cauchy priors to see how big the effect from updating on one data point can be even with relatively uninformative priors.

The results of our Bayesian analysis can be found in Tables \ref{tab:other-domains-results-beta-lambda-table} and \ref{tab:other-domains-results-returns-table}. Figure \ref{fig:other-domains-results-returns-violin} shows the posterior distributions we obtain over the returns to software R\&D parameter \( r = \lambda/\beta \) in a more accessible violin plot format.

\begin{table}[H]
\centering
\small
\begin{tabular}{@{}lll@{}}
\toprule
                     & $ \beta $                    & $ \lambda $  \\
\midrule
Computer vision      & 0.824 (0.203 to 3.27)        & 1.11\;\: (0.186 to 4.92) \\
RL sample efficiency & 0.883 (0.205 to 2.99)        & 1.14\;\: (0.108 to 5.36) \\
SAT solvers          & 0.600 (0.153 to 2.28)        & 1.58\;\: (0.154 to 8.93) \\
Linear programming   & 1.24\;\: (0.260 to 3.93)     & 0.944 (0.0845 to 4.46) \\
\bottomrule
\end{tabular}
\caption{Estimates of \( \beta \) and \( \lambda \) according to their posterior distributions across categories. We report the median as the point estimate outside parentheses and the central 90\% confidence interval (5th to 95th percentiles) in parentheses.}
\label{tab:other-domains-results-beta-lambda-table}
\end{table}

The results in Table \ref{tab:other-domains-results-beta-lambda-table} may initially be rather hard to interpret, so it's useful to keep what we would obtain from just the prior distribution of half Cauchy with unit scale. The quantile function of the half Cauchy distribution with unit scale is \( Q(\alpha) = \tan(\alpha \pi/2) \), so if we just used the prior for \( \beta, \lambda \) without any Bayesian update, we would expect to get a median of 1 with a 90\% confidence interval of \( \tan(0.05 \cdot \pi/2) \approx 0.078 \) to \( \tan(0.95 \cdot \pi/2) \approx 12.7 \). Looking at the results in Table \ref{tab:other-domains-results-beta-lambda-table}, the Bayesian update narrows the distribution of the parameters relative to this baseline in all cases, though the updates on \( \beta \) are stronger than those on \( \lambda \).

\begin{table}[H]
\centering
\small
\begin{tabular}{@{}llllll|l@{}}
\toprule
                     & 5th    & 25th  & \textbf{50th}  & 75th  & 95th & Naive estimate \\
\midrule
Computer vision      & 0.528  & 1.15  & \textbf{1.40}  & 1.57  & 2.26 & 1.45 \\
RL sample efficiency & 0.168  & 0.775 & \textbf{1.44}  & 2.01  & 4.20 & 1.66 \\
SAT solvers          & 0.415  & 1.76  & \textbf{3.02}  & 4.00  & 6.41 & 4.17 \\
Linear programming   & 0.0833 & 0.410 & \textbf{0.851} & 1.39  & 3.39 & 1.51 \\
\bottomrule
\end{tabular}
\caption{Percentiles of the posterior distribution of the returns to software parameter \( r \) across categories. The posterior medians are in bold. The naive estimate column reports the results of estimating \( r \) by dividing the growth rates of the outputs and the inputs as explained in Section \ref{sec:naive-method}.}
\label{tab:other-domains-results-returns-table}
\end{table}

The narrowing of the distribution is even more pronounced in Table \ref{tab:other-domains-results-returns-table}. This is because the prior for \( r \) is the ratio of two independent half-Cauchy random variables with unit scale and because the half-Cauchy distribution is invariant under taking reciprocals, so the prior for \( r \) is the distribution of the product of two independent half-Cauchy random variables with unit scale, which is identical to the distribution of \( |XY| \) where the variables \( X, Y \) are independent and Cauchy with unit scale. This distribution can be inferred from the results in \cite{springer1966distribution} and has density

\[ f_{\text{half cauchy product}}(x) = \frac{4}{\pi^2} \frac{\log x}{x^2 - 1} \]

on the positive real numbers. Numerical integration then gives us that the prior distribution for \( r \) has a median of \( 1 \) (this is obvious from the \( x \to 1/x \) symmetry) and a 90\% confidence interval of  \( 0.0267 \) to \( 37.5 \). This interval is roughly three orders of magnitude wide, and in all cases, we observe a substantial reduction of this prior uncertainty after performing a Bayesian update on a single data point.

\begin{figure}[H]
\centering
\includegraphics[scale=0.75]{visuals/returns_violin_plot.pdf}
\caption{Violin plot of the posterior distributions we obtain for the parameter \( r \) across categories. The kernel density plots are restricted to the \( 99\%\) confidence interval for accessibility; in fact, they have heavier tails than are visible in the plot.}
\label{fig:other-domains-results-returns-violin}
\end{figure}
